Your "Pro" LLM Subscription May Actually Be "Free": Exposing Fingerprint Spoofing Risks in LLM Inference Services

As Large Language Model (LLM) APIs become ubiquitous, users increasingly rely on black-box fingerprinting to verify that providers are serving the advertised premium models. However, these methods may overlook adversarial providers who manipulate model weights to cheat the fingerprint process. We introduce a novel threat termed fingerprint spoofing, where a malicious provider stealthily serves a weaker model that has been parameter-efficiently fine-tuned to mimic a stronger model, thereby evading user-side fingerprinting. We first formally prove that user-side resource constraints (i.e., finite query budgets and weak fingerprinting classifiers) make current fingerprinting vulnerable to fingerprint spoofing. Guided by this theoretical analysis, we propose GhostPrint, a cost-effective attack framework leveraging surrogate modeling, reward-ranked fine-tuning, and knowledge distillation. Extensive evaluations in both static and continual fingerprinting settings demonstrate that GhostPrint allows weak models to consistently bypass representative fingerprint methods while maintaining utility at a low fine-tuning cost, exposing a critical vulnerability in current LLM fingerprinting pipelines.

==> __append_toc.tex <==

%\usepackage{enumitem}

\makeatletter

% Will store the items for the appendix list of contents
\newcommand{\applist}{}

% Ignore stale aux entries from the old version:
% \@addtoapplist{title}{label}
\newcommand{\@addtoapplist}[2]{}

% Called when reading from the .aux to actually build \applist
\newcommand{\@addtoapplistnumber}[3]{%
  % #1 = section number
  % #2 = section title
  % #3 = hyperlink anchor
  \g@addto@macro\applist{%
    \item \textbf{Section~\hyperlink{#3}{#1}}: #2.%
  }%
}

% Called when defining a new appendix section: writes to .aux
\newcommand{\addtoapplist}[1]{%
  \begingroup
    \edef\appsecnum{\thesection}%
    \edef\appanchor{appsec.\thesection}%
    \protected@write\@auxout{}{%
      \string\@addtoapplistnumber{\appsecnum}{#1}{\appanchor}%
    }%
  \endgroup
}

% Wrapper: use this instead of \section in the appendix
\newcommand{\appsection}[1]{%
  \section{#1}%
  \hypertarget{appsec.\thesection}{}%
  \addtoapplist{#1}%
}

\makeatother
